Extending INLA to a class of near-Gaussian latent models

This work extends the Integrated Nested Laplace Approximation (INLA) method to latent models outside the scope of latent Gaussian models, where independent components of the latent field can have a near-Gaussian distribution. The proposed methodology is an essential component of a bigger project that aim to extend the R package INLA (R-INLA) in order to allow the user to add flexibility and challenge the Gaussian assumptions of some of the model components in a straightforward and intuitive way. Our approach is applied to two examples and the results are compared with that obtained by Markov Chain Monte Carlo (MCMC), showing similar accuracy with only a small fraction of computational time. Implementation of the proposed extension is available in the R-INLA package.

==> fig/ngnodes-concordance.tex <==
\Sconcordance{concordance:inla_ngnodes_revised.tex:inla_ngnodes_revised.Rnw:%
1 450 1 1 14 553 1}

